How many bots are you following?

Social Media are evolving as a pervasive source of news able to reach a larger audience through their spreading power. The main drawback is given by the presence of malicious accounts, known as social bots, which are often used to diffuse misleading information. Social bots are automated accounts whose goal is to interact with humans and influence them. Starting from the definition of credulous (i.e., human accounts with a high percentage of bot friends among their followees, in this work we aim to single out a regression model to derive, with an acceptable margin of error, the percentage of bot-followees of a human-operated account. The advantage lies in knowing, as a preventive measure, which users may be the target of bots' activities, hence more exposed to the misleading/unreliable content. Our results showed that the best regression model achieves a Mean Absolute Error of 3.62% and a Root Mean Squared Error of 5.96%, thus encouraging further research in this direction.

==> sections/5.3-table_Cred443.tex <==
\begin{table}[H]
	\begin{centering}
		\begin{tabular}{lccc}
		\hline
		\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{3}{c}{\textbf{Feature sets}}\\
		\cline{2-4}
		& \textit{Botometer}+ & \textit{ClassA-} & \textit{All\_features} \\
		\hline
		$\rightarrow$ ZeroR $\leftarrow$ (baseline) &  &  &  \\
        REPTree & 6.95 & 6.84 & 6.37 \\
        LinearRegression & 6.38 & 7.20 & 7.07 \\
        IBk & 8.31 & 7.91 & 8.22 \\
        LWL & 6.34 & 6.57 & 6.45 \\
        AdditiveRegression & 6.26 & 6.04 & 5.93 \\
        RegressionByDiscretization & 7.84 & 7.34 & 8.47 \\
        M5Rules & 6.81 & 7.17 & 8.38 \\
        DecisionStump & 6.28 & 6.47 & 6.47 \\
        GaussianProcesses & 6.37 & 7.01 & 6.73 \\
        SMOreg & 6.55 & 7.00 & 6.65 \\
        MultilayerPerceptron & 8.26 & 9.01 & 11.06 \\
        MLPRegressor & 8.21 & 7.35 & 8.07 \\
        RandomForest & 6.40 & 6.03 & 5.96 \\
		\hline
		\end{tabular}
		\caption{RMSE regression}
		\label{tab:rmse_cred443}
	\end{centering}
\end{table}

\begin{table}[H]
	\begin{centering}
		\begin{tabular}{lccc}
		\hline
		\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{3}{c}{\textbf{Feature sets}}\\
		\cline{2-4}
		& \textit{Botometer}+ & \textit{ClassA-} & \textit{All\_features} \\
		\hline
		$\rightarrow$ ZeroR $\leftarrow$ (baseline) & 6.68 & 6.68 & 6.68 \\
        REPTree & 4.73 & 4.50 & 4.40 \\
        LinearRegression & 4.51 & 4.72 & 4.56 \\
        IBk & 5.45 & 5.11 & 5.38 \\
        LWL & 4.41 & 4.49 & 4.46 \\
        AdditiveRegression & 4.43 & 4.27 & 4.17 \\
        RegressionByDiscretization & 5.31 & 4.86 & 5.50 \\
        M5Rules & 4.67 & 4.72 & 4.84 \\
        DecisionStump & 4.40 & 4.51 & 4.51 \\
        GaussianProcesses & 4.54 & 4.66 & 4.56 \\
        SMOreg & 4.16 & 4.28 & 4.13 \\
        MultilayerPerceptron & 5.64 & 6.14 & 6.79 \\
        MLPRegressor & 5.29 & 4.72 & 5.04 \\
        RandomForest & 4.63 & 4.26 & 4.33 \\
		\hline
		\end{tabular}
		\caption{MAE regression}
		\label{tab:mae_cred443}
	\end{centering}
\end{table}

==> sections/5.4-table_Cred502.tex <==
\begin{table}[H]
	\begin{centering}
		\begin{tabular}{lccc}
		\hline
		\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{3}{c}{\textbf{Feature sets}}\\
		\cline{2-4}
		& \textit{Botometer}+ & \textit{ClassA-} & \textit{All\_features} \\
		\hline
		$\rightarrow$ ZeroR $\leftarrow$ (baseline) & 6.57 & 6.57 & 6.57 \\
        REPTree & 6.27 & 6.34 & 6.73 \\
        LinearRegression & 6.27 & 6.49 & 6.14 \\
        IBk & 7.91 & 8.10 & 8.22 \\
        LWL & 6.14 & 6.54 & 6.43 \\
        AdditiveRegression & 6.28 & 6.27 & 5.98 \\
        RegressionByDiscretization & 7.42 & 6.50 & 7.42 \\
        M5Rules & 6.47 & 7.18 & 7.26 \\
        DecisionStump & 6.16 & 6.62 & 6.66 \\
        GaussianProcesses & 6.24 & 6.56 & 6.14 \\
        SMOreg & 6.47 & 6.74 & 6.26 \\
        MultilayerPerceptron & 9.01 & 7.76 & 9.91 \\
        MLPRegressor & 8.11 & 7.17 & 8.72 \\
        RandomForest & 6.21 & 6.05 & 5.99 \\
		\hline
		\end{tabular}
		\caption{RMSE regression}
		\label{tab:rmse_cred502}
	\end{centering}
\end{table}

\begin{table}[H]
	\begin{centering}
		\begin{tabular}{lccc}
		\hline
		\multirow{2}{*}{\textbf{Algorithms}} & \multicolumn{3}{c}{\textbf{Feature sets}}\\
		\cline{2-4}
		& \textit{Botometer}+ & \textit{ClassA-} & \textit{All\_features} \\
		\hline
		$\rightarrow$ ZeroR $\leftarrow$ (baseline) & 4.51 & 4.51 & 4.51 \\
        REPTree & 4.41 & 4.46 & 4.45 \\
        LinearRegression & 4.39 & 4.46 & 4.27 \\
        IBk & 5.21 & 5.28 & 5.26 \\
        LWL & 4.25 & 4.45 & 4.43 \\
        AdditiveRegression & 4.40 & 4.27 & 4.09 \\
        RegressionByDiscretization & 4.99 & 4.55 & 5.09 \\
        M5Rules & 4.45 & 4.67 & 4.51 \\
        DecisionStump & 4.29 & 4.57 & 4.60 \\
        GaussianProcesses & 4.40 & 4.41 & 4.27 \\
        SMOreg & 4.08 & 4.08 & 3.96 \\
        MultilayerPerceptron & 6.16 & 4.94 & 6.49 \\
        MLPRegressor & 5.10 & 4.67 & 5.10 \\
        RandomForest & 4.50 & 4.23 & 4.28 \\
		\hline
		\end{tabular}
		\caption{MAE regression}
		\label{tab:mae_cred502}
	\end{centering}
\end{table}
